DIMON: Learning Solution Operators of Partial Differential Equations on a Diffeomorphic Family of Domains

The solution of a PDE over varying initial/boundary conditions on multiple domains is needed in a wide variety of applications, but it is computationally expensive if the solution is computed de novo whenever the initial/boundary conditions of the domain change. We introduce a general operator learning framework, called DIffeomorphic Mapping Operator learNing (DIMON) to learn approximate PDE solutions over a family of domains $\{\Omega_{\theta}}_\theta$, that learns the map from initial/boundary conditions and domain $\Omega_\theta$ to the solution of the PDE, or to specified functionals thereof. DIMON is based on transporting a given problem (initial/boundary conditions and domain $\Omega_{\theta}$) to a problem on a reference domain $\Omega_{0}$, where training data from multiple problems is used to learn the map to the solution on $\Omega_{0}$, which is then re-mapped to the original domain $\Omega_{\theta}$. We consider several problems to demonstrate the performance of the framework in learning both static and time-dependent PDEs on non-rigid geometries; these include solving the Laplace equation, reaction-diffusion equations, and a multiscale PDE that characterizes the electrical propagation on the left ventricle. This work paves the way toward the fast prediction of PDE solutions on a family of domains and the application of neural operators in engineering and precision medicine.

==> backup.tex <==
%% many query problems in engineering and medicine
Heavy computational burden induced by solving many-query partial differential equations (PDEs) impedes a broader adoption of computational models in both engineering and medicine. 

%% learning operator
The emerging field of artificial intelligence has profoundly influenced the approaches for solving PDEs. Common approaches, represented by physics-informed neural networks~\cite{lu2021deepxde,karniadakis2021physics,cai2021physics,hao2023pinnacle}, deep Ritz method~\cite{yu2018deep}, and deep Galerkin method~\cite{sirignano2018dgm}, approximate PDE solutions with neural networks at one instance with fixed boundary conditions (BCs) and initial conditions (ICs). However, the need for retraining under various ICs and BCs has greatly limited the applicability of these approaches. Neural operators have been developed to overcome this issue, where neural networks are trained to directly learn the solution operator, thereby can approximating PDE solutions given various ICs, BCs, and local material properties, etc.~\cite{lu2021learning,li2020fourier,jiang2023fourier,zhu2023fourier}. Despite the initial successes, operator learning is still limited to a fixed domain, where even a slight change in the learning domain leads to network retraining. There are a few works that have addressed this issue: Geometry-aware Fourier Neural Operator (Geo-FNO)~\cite{li2022geoFNO} concatenated two networks prior to and posterior to the FNO model~\cite{li2020fourier} for transforming a mesh on an irregular back to a uniform mesh due to the nature of fast Fourier transform (FFT)-based learning. However, the stringent assumption of mapping back to a square domain is yet to be addressed for non-diffeomorphic shapes. Another work utilizes deep operator networks (DeepONets) in airfoil shape optimization~\cite{shukla2023deep}; however, the problem setup is inconsistent with the theorem proposed in~\cite{lu2021learning,jin2022mionet}, which requires learning on a fixed compact set. He et al.~\cite{he2023novel} applied a U-Net structure with convolutional neural networks (CNN) to encode geometric information of 2D structures to the latent space.


The critical challenge of learning on a family of geometries $\{\Omegatheta\}_{\theta\in\Theta}$ emanates from learning functional mapping on a family of Banach spaces. That is, the PDE solution essentially is approximated on a distinctive Banach space if the computational domain varies, even if the function form of the PDE remains the same. Therefore, learning the solution operator on various domains is equivalent to learning a family of operators posed on various $\Omegatheta$. Yang et al.~\cite{yang2023context} addressed the issue of learning multi-operators by proposing an in-context operator learning (``ICON") that utilizes few-shot learning to approximate the solutions operators for PDEs with different functional forms. 

In this work, we propose a learning framework that transforms the problem of learning a family of operators to learning a single latent operator parameterized by domain shapes on a unified reference domain (``template") $\Omegaref$. This simplified problem setup is compatible with most of the current operator learning networks~\cite{lu2021learning,li2020fourier,seidman2022nomad,zhu2023reliable}. The idea is inspired by the notion of functional maps in computer vision~\cite{ovsjanikov2012functional}. PDE solutions along with initial/boundary conditions on a family of topologically equivalent shapes are mapped through a bijective $C^{2}$ mapping onto a reference domain (pushforward) with the original shape being parameterized. Then, a neural operator is trained to learn the solution operator of a latent PDE on the reference domain $\Omegaref$. The final step is to perform a pullback of the predicted PDE solution to the original domain. Thus, learning PDE operators in parametric domains is completed. Notice that the operator of the latent PDE on $\Omegaref$ is a ``counterpart" to the original PDE operator and can approximate the original operator composited with a pullback. 

Notably, efficient shape parameterization is a critical question to be addressed in our framework. Shape can be expressed in various common representations, such as mesh, point clouds, and voxels, albeit these representations are high-dimensional. However, learning with these high-dimensional representations is challenging in network training. Notably, methods developed in statistical shape analysis~\cite{dryden2016statistical} can serve as promising candidates for effectively projecting the representation of a complicated shape onto a low dimension as ``shape parameter" using methods developed in dimensionality reduction, i.e., principal component analysis (PCA)~\cite{stegmann2002brief}. 

To facilitate dimensionality reduction, we calculate point correspondence across all geometries with the reference domain and perform PCA on the landmark points for their distances in Euclidean space. One can easily calculate the shape parameter for parameterized shapes when the point correspondence is known. However, one rarely encounters parameterized shapes with rigid mesh settings using realistic data, which motivates the development of numerous approaches of calculating point correspondences for unparameterized shapes where the point correspondence is not known a priori~\cite{masci2015geodesic,chui2000new,ovsjanikov2016computing,cates2017shapeworks}. We demonstrate the ability of our framework with three examples, which contain learning static and dynamic problems on parameterized domains and predicting electrical propagation on unparameterized left ventricles (LVs). For the last example, one could adopt the aforementioned approaches to calculate registration across various geometries. However, we identify the point correspondence by matching the universal ventricular coordinates (UVCs) due to the special structure of the LV~\cite{sung2022fat,reuter2006laplace}.

%% organization
% The remainder of this manuscript is organized as follows. In Sec.~\ref{subsec:prob_formul}, we formulate the learning framework and show that a current neural operator is able to learn the operator on various geometries (Sec.~\ref{subsec:theorem}). Then, we present several examples in Sec.~\ref{subsec:lap}-\ref{subsec:LV}. A summary of the benchmarks is presented in Table~\ref{table:example}. We conclude with a discussion and future directions in Sec.~\ref{sec:disc}.



\begin{table}
\centering
\small
\begin{adjustbox}{}%{width=0.4\textwidth}
 \begin{tabular}{ c | c c c } 
 \hline
 Examples & Equation & Shape Generation & reference domain $\Omegaref$ \\
 \hline
 2D Laplace & $\Delta u = 0$  &  Synthetic  & Square  \\
 2D Reaction Diffusion & $u_{t} = \Delta u + f(u, r)$  & Synthetic & Annulus \\
 3D Electrophysiology & $C_{m}u_{t} = -(I_{ion} + I_{stim}) + \nabla D \nabla u $ & MRI & Hollow Semi-Sphere \\
 \hline
\end{tabular}
\end{adjustbox}
\caption{ \textbf{Summary of examples for assessing the performance of the operator learning for predicting PDEs posed on different geometries.} }
\label{table:example}
\end{table}
